Verified Parallel String Matching in Haskell

In this paper, we prove correctness of parallelizing a string matcher using Haskell as a theorem prover. We use refinement types to specify correctness properties, Haskell terms to express proofs and Liquid Haskell to check correctness of proofs. First, we specify and prove that a class of monoid morphisms can be parallelized via parallel monoid concatenation. Then, we encode string matching as a morphism to get a provably correct parallel transformation. Our 1839LoC prototype proof shows that Liquid Haskell can be used as a fully expressive theorem prover on realistic Haskell implementations.

==> distribution.tex <==
\section{String Matching Distributes over Input}\label{sec:distribution}
%
In this section we prove that String Matching distributes over @RString@.
%
We first (\S~\ref{subsec:toSM}) we define the functino @toSM::RString -> SM target@
that creates a String Matcher for its input String, 
and then (\S~\ref{subsec:distribution:sm}) we prove distribution of @toSM@ over mappend. 
%
Next, we will use this proof combined with the Theorem of 
Distribution over monoid concatenation (\S~\\ref{sec:monoid:distribution}), 
to prove that String Matching Distributes over Monoid Concatenation.

\subsection{Distribution of String Matching over Strings}\label{subsec:toSM}

The function @toSM input@  creates a String Matcher @SM target@
structure that matches the type level string target to the 
string value argument @input@.
\begin{code}
toSM :: forall (target :: Symbol). (KnownSymbol target) 
     => RString -> SM target 
toSM input = SM input (makeSMIndices input tg) 
  where
    tg = fromString (symbolVal (Proxy :: Proxy target))
\end{code}
%
The input field of the result is the input string, 
while the indices are computed by calling @makeIndices@ 
in the range from @0@ to @stringLen input -1@
via @makeSMIndices@
%
\begin{code}
makeSMIndices 
  :: input:RString -> target:RString 
  -> [GoodIndex input target]
makeSMIndices input target 
  = makeIndices input target 0 (stringLen input - 1)
\end{code}

\subsection{Distribution of String Matching over Refined Strings}\label{subsec:distribution:sm}

Next, we prove that @toSM@ distributes over mappending
\begin{theorem}[Distribution of string matching]\label{theorem:distribution:toSM}
\begin{code}
distributestoSM :: x:RString -> y:RString 
  -> { toSM x mappend toSM y == toSM (x stringMappend y)}
\end{code}
\end{theorem}

\begin{proof}
The core of the proof starts from the left hand side 
creating two matching structures, one for each input 
substring @x@ and @y@. 
%
The mappending of these two string matchers leads to 
three set of indices
1. @xis@ from the input @x@, 
2. @xyis@ from mappending the two strings, and
3. @yis@ from the input @y@.
%
We prove using lemmata, 
that appending these three sets of indices is equal to 
the indices directly created from the mappended input @x stringMappend y@.
\begin{code}
distributestoSM x y 
  =   (toSM x :: SM target) <> (toSM y :: SM target)  
  ==. (SM x is1) <> (SM y is2)
  ==. SM i (xis ++ xyis ++ yis)
  ==. SM i (makeIndices i tg 0 hi1 ++ yis) 
      ?  (mapCastId tg x y is1 
      &&& mergeNewIndices tg x y)
  ==. SM i (makeIndices i tg 0       hi1 
         ++ makeIndices i tg (hi1+1) hi) 
      ? shiftIndicesRight 0 hi2 x y tg 
  ==. SM i is
      ? mergeIndices i tg 0 hi1 hi
  ==. toSM (x <+> y)
  *** QED 
  where
    xis  = map (castGoodIndexRight tg x y) is1
    xyis = makeNewIndices x y tg
    yis  = map (shiftStringRight   tg x y) is2

    tg  = fromString (symbolVal (Proxy::Proxy target))
    is1 = makeSMIndices x tg 
    is2 = makeSMIndices y tg 
    is  = makeSMIndices i tg 

    i = x <+> y

    hi1 = stringLen x - 1
    hi2 = stringLen y - 1
    hi  = stringLen i - 1 
\end{code}
%
The proof uses four lemmata.
Identity of casting @mapCastId@
is reused and explained in the associativity proof. 
Here we explain the rest three
\begin{itemize}
\item Merging indices from low to high, using some medium value
\begin{code}
mergeIndices 
  :: input:RString -> target:RString 
  -> lo:Nat -> mid:{Int | lo <= mid} 
  -> hi:{Int | mid <= hi} 
  -> { makeIndices input target lo hi   == 
      makeIndices input target lo mid  ++ 
      makeIndices input target (mid+1) hi} 
\end{code}
The lemma states that making indices for the strings @input@ and @target@
in the range from @lo@ to @hi@
is equivalent to makeing indices for the same string in the ranges
from @lo@ to @mid@ appended with the range from @mid+1@ to @hi@, 
for any @mid@ between @lo@ and @hi@. 
%
The proof of the lemma proceeds by induction on @mid@.

\item Merging the indices of the first substring
\begin{code}
mergeNewIndices 
  :: tg:RString -> x:RString -> y:RString
  -> { makeSMIndices x tg 
    ++ makeNewIndices x y tg
    == makeIndices (x <+> y) tg 0 (lenStr x - 1)} 
\end{code}
The theorem states that appending the indices that appear in the first string @x@, 
that is the indices @xis@ that do not and the indices @xyis@ that do involve @y@, 
is equivalent to the indices @is@ on the input @x stringMappend y@
in the range from @0@ to @lenStr x -1@. 
%
The proof case splits on the sizes of @tg@ and @x@. 
%
If the size of the target is less than two, then @xyis@ is empty, 
but @xis == is@, as appending @y@ to the input cannot create more indices. 
%
Otherwise, if the input @x@ is smaller than the target, 
then @xis@ is empty and @xyis@ is equal to @is@. 
%
Otherwise, we set @mid = stringLen x1 - stringLen tg@ 
and use the previous @mergeIndices@ lemma to merge @xis@ and @yis@ into @is@.
\item Shifting is left concatenation.
\begin{code}
shiftIndicesRight
  :: lo:Nat -> hi:Int  
  -> x:RString -> y:RString 
  -> tg:RString
  -> { map (shiftStringRight tg x y) 
           (makeIndices y tg lo hi) 
  == makeIndices (x stringMappend y) tg 
                 (lenStr x + lo) (lenStr x + hi) }

\end{code}
The lemma states that shifting indices from @lo@ to @hi@ on @y@
is equivalent to computing the indices from @lenStr x + lo@
to @lenStr x + hi@ on @x stringMappend y@, 
and it is proved by induction on the difference @hi - lo@.
\end{itemize}
\qed\end{proof}




==> monoid-distribution.tex <==
\section{Verification of Distribution over Monoid Concatenation}~\label{sec:monoid:distribution}
In this section we prove distribution over monoid concatenation. 
%
Concretely, if a function @f :: i -> m@
from some input @i@ to a monoid @m@, 
distributes on the input
@f (i1 stringMappend i2) == (f i1) mappend (f i2)@, 
then @f@ distributes over monoid concatenation: 
@f i == mconcat (map f (chunk n i))@. 
%
For the above property to hold, the input @i@
should satisfy certain properties, 
for example, the input should define the methods
@stringMappend@ and @chunk@. 
%
First~\S~\ref{subsec:rstring} we defined Refined Strings 
as an example of proper inputs, and then~\S~\ref{subsec:distribution}
we prove distribution over Monoid Concatenation on Refined Strings.  


\subsection{Refined Strings}\label{subsec:rstring}
We represent the input as a Refined String 
defined at a library @RString.hs@
with implementation irrelevant for the proofs.  
%
\NV{introduce RString here is good, but implementation and constact time indexing seems irrelevant here}
\begin{code}
data RString
\end{code}
%
@RString.hs@
defines the monoid operators @stringMempty@ and @(stringMappend)@
that satisfy the monoid laws. 
%
Moreover, it defines string manipulation operators
that come refined via various theorems. 
%
For example, the library exposes the
operators @takeStr@ and @dropStr@
\begin{code}
takeStr :: i:Nat -> xs:{RString | i <= stringLen xs } 
  -> {v:RString | stringLen v == i }
dropStr :: i:Nat -> xs:{RString | i <= stringLen xs } 
  -> {v:RString | stringLen v == stringLen xs - i}
\end{code}
%
and asserts that appending a list split via @take@ and @drop@
exactly reconstructs the list.
\begin{code}
concatTakeDrop 
  :: i:Nat -> xs:{RString | i <= stringLen xs} 
  -> {xs == takeStr i xs stringMappend dropStr i xs }
\end{code}
%
The operators defined in @RString@ are already reflected in the logic. 
%
Thus we use them to further define operators
that we reflect and use in the theorems. 
%
For example, @takeStr@ and @dropStr@ are used to define 
@chunkStr@ 
\begin{code}
chunkStr i xs 
  | i <= 1 ||stringLen xs <= i 
  = C xs N 
  | otherwise
  = C (takeStr i xs) (chunkString i (dropStr i xs))
\end{code}
%
We reflect @chunkStr@ into logic and use it to define and prove 
distribution over monoid concatenation. 


\subsection{Distribution over Monoid Concatenation on Refined Strings}\label{subsec:distribution}
%
We use the refinement type specification for @monoidDirstibution@
to specify and prove  that for each monoid @m@, 
if the function @f:RString -> m@ distributes over @RString@
then it distributes over monoids. 
%
Note that the assumption of the theorem, 
is expressed in the specifications as a functional argument 
that makes the proper assumptions for @f@. 
%
To prove distribution over monoids for a specific @f@, 
we need to invoke @monoidDirstibution@ 
on @f@ and a proper proof argument that @f@ distributes over @RString@.
%
\begin{theorem}[Monoid Distribution]\label{theorem:monoid:distribution}
If @m@ is a monoid, then each function @f:RString -> m@
that distributes over @RString@, distributes over monoid concatenation.
%
\begin{code}
monoidDirstibution
  :: f:(RString -> m)
  -> (x1:_ -> x2:_ -> {f (x1 stringMappend x2) == (f x1) <> (f x2)} )
  -> is:RString
  -> n:Int 
  -> {f is == mconcat (map f (chunkStr n is))}
\end{code}
\end{theorem}

\begin{proof}
The proof proceeds by induction on the length of the input.
%
\begin{code}
monoidDirstibution f thm is n  
  | stringLen is <= n || n <= 1
  =   mconcat (map f (chunkStr n is))
  ==. mconcat (map f (C is N))
  ==. mconcat (f is `C` map f N)
  ==. f is <> mconcat N
  ==. f is <> mempty 
  ==. f is ? idRight (f is)
  *** QED 
monoidDirstibutionf f thm is n  
  =   mconcat (map f (chunkStr n is))
  ==. mconcat (map f (C takeIs (chunkStr n dropIs))) 
  ==. mconcat (f takeIs `C` map f (chunkStr n dropIs))
  ==. f takeIs <> f dropIs
       ? monoidDirstibution f thm dropIs n  
  ==. f (takeIs <+> dropIs)
       ? thm takeIs dropIs
  ==. f is 
       ? concatTakeDrop n is 
  *** QED  
  where
    dropIs = dropStr n is 
    takeIs = takeStr n is 
\end{code}
%
In the base case we use rewriting and right identity on the monoid @f is@. 
%
In the inductive case, 
we use the inductive hypothesis on the input @dropIs = dropStr n is@, 
that is provably smaller than @is@ as @n > 1@. 
%
Then, by our assumption argument @thm takeIs dropIs@
we get basic distribution of @f@, that is 
@f takeIs <> f dropIs == f (takeIs stringMappend dropIs)@. 
%
Finally, we merge @takeIs stringMappend dropIs@ to @is@
using the property @concatTakeDrop@ take is exported by the @RString@
library.
\qed\end{proof}

==> monoid.tex <==
\section{Dependent Type String Indexing is a Monoid}\label{sec:monoid}



\subsection{String Matching Definition}

We define the String Matching data type
@SM target@ to contain a string field @input@ and
a list of all the indices on @input@ where the
@target@ appears.
%
\begin{code}
data SM (target :: Symbol) where
  SM :: input:RString
     -> indices:[GoodIndex input target]
     -> SM target
\end{code}
%
We used type literals to parameterize the type over
the Symbol @target@.
%
This encoding is required to allow definition of
an identity element, as explained later~(\S~\ref{subsec:monoid:methods}).
%
The input field, of type @RString@, is a refined wrapper on
a String manipulation library that
1. allows for constant time string indexing, and
2. provides various string lemmata.
%
The library @RString.hs@~\footnote{
\href{https://github.com/nikivazou/verified_string_indexing/blob/master/src/String.hs}
     {\url{https://github.com/nikivazou/verified_string_indexing/blob/master/src/String.hs}}}
implements @RString@ as @ByteStrings@,
and \textbf{assumes} various String properties,
like left identity:
\begin{code}
assume leftIdentity :: s:RSTring -> { s <+> stringMempty == s }
\end{code}
%
The indices field is a list of good indices.
%
For simplicity we are using Haskell's built in lists but in the
implementation we use a user defined reflected list data type similar
to that presented in section~\ref{sec:haskell-proofs}.
%
A @GoodIndex input target@ is a refined type alias
for an integer @i@ that
1. is a natural number,
2. @target@ is a substring of @input@ appearing at position @i@.
%
\begin{code}
type GoodIndex Input Target
  = {i:Nat | isGoodIndex Input (fromString Target) i }

isGoodIndex :: RSTring -> RSTring -> Int -> Bool
isGoodIndex input target i
  =  (subString input i (stringLen target)  == target)
  && (i + stringLen target <= stringLen input)
\end{code}
%

As an example, the good indices of @"abcab"@ on @"ababcabcab"@
are @[2,5]@ while any other index is bad.
\begin{code}
goodSM :: SM "abcab"
goodSM = SM "ababcabcab" [2, 5]

badSM  :: SM "abcab"
badSM  = SM "ababcabcab" [0, 7]
\end{code}
\NV{Liquid Haskell actually will reject both the above, as the stringLen and subString functions are uninterpreted}

\subsection{Monoid Laws}
In the rest of this section we will prove that
the String Matching structure is a Monoid.
%
A structure @m@ is a monoid,
there is an identity element @mempty :: a@
and an associative appending function @(<>) :: a -> a -> a@.
That is, @mempty@ and @(<>)@ should satisfy the following laws
\begin{figure}
\begin{code}
idLeft :: x:a -> {x <> mempty == x }
idRight:: x:a -> {mempty <> x == x }
assoc  :: x:a -> y:a -> z:a -> {(x <> y) <> z == x <> (y <> z)}
\end{code}
\caption{Monoid Laws}
\label{fig:monoid:laws}
\end{figure}
%
To prove that the String Matching operator @SM@
is a monoid, we use the fact that the String and list
of indices contained in its fields are also monoids.
%
Figure~\ref{fig:monoids} defines the monoid operators used
in this section.
%
\begin{figure}
$$
\begin{array}{c c c c }
\text{Structure} & \text{Identity} & \text{Mappend} & \text{Laws} \\
\hline
\texttt{List} & \listMempty & (\listMappend) & \text{PROVEN} \\
\texttt{SM} & \mempty & (\mappend) & \text{PROVEN} \\
\texttt{RString} & \stringMempty & (\stringMappend) & \text{ASSUMED}
\end{array}
$$
\caption{Monoid Structures}
\label{fig:monoids}
\end{figure}


\subsection{Monoid Methods for String Matching}~\label{subsec:monoid:methods}
Next, we define the mappend and identity elements for string matching.
We reflect the definitions into logic, to latter use them to prove
the monoid laws.

The \textit{identity element} of @SM t@, for each target @t@, is
defined to contain the identity @RString@ (@stringMempty@) and the
identity @List@ (@listMempty@).
\begin{code}
reflect mempty
mempty:: forall (t :: Symbol). SM t
mempty = SM stringMempty listMempty
\end{code}
%
Note, that if target was encoded as a value argument, instead of a
type parameter, then there would be no way to define an identity
element for each expression argument.
%
\JP{I think the type parameter is more necessary to define mappend}


The @(mappend)@ operator,
mappends the two input strings.
The appended indices, as depicted in Figure~\ref{fig:mappend:indices},
are the concatenations of three list indices:
\begin{enumerate}
\item The indices @is1@ from the first input, casted to be good indices in the new structure,
\item the new indices @newIs@ created when concatenating the two strings, and
\item the indices @is2@ from the second input, shifted right @stringLen i2@ points.
\end{enumerate}
%
\begin{figure}
\includegraphics[scale=0.5]{makeIndices}
\caption{Mappend indices of String Matcher}
\label{fig:mappend:indices}
\end{figure}
%
The above are summarized in the Haskell definition of @(<>)@
\begin{code}
reflect mappend
(mappend)::forall (t::Symbol). KnownSymbol t => SM t -> SM t -> SM t
(SM i1 is1) mappend (SM i2 is2)
  = SM (i1 stringMappend i2) (is1' listMappend newIs listMappend is2')
  where
    tg    = fromString (symbolVal (Proxy :: Proxy t))
    is1'  = map (castGoodIndexLeft tg i1 i2) is1
    newIs = makeNewIndices i1 i2 tg
    is2'  = map (shiftStringRight tg i1 i2) is2
\end{code}

\paragraph{Step 1: Casting Good Indices}
If @is@ is a list of good indices for string @i1@ with respect to a target @tg@,
then @is@ is a list of good indices for the string @i1 stringMappend i2@, for each @i2@
for the same target.
%
To establish the above property,
we need the property from refined string
that states that
for each string @input@ and @input'@
and each integers @i@ and @j@ whose sum does not exceed the length of @input@,
the @subString@ on @input@ from @i@ with length @j@
is equal to
the @subString@ on @input stringMappend input'@ from @i@ with length @j@:
%
\begin{code}
subStringConcatLeft
    :: sl:RString -> sr:RString -> j:Int
    ->  i:{Int | i + j <= stringLen sl }
    ->  { subString sl i j == subString (sl stringMappend sr) i j }
\end{code}
%
To cast an index list of good indices in the above way,
we cast the above property to every element of the list
%
\begin{code}
reflect castGoodIndexRightList
castGoodIndexLeft
  :: tg:RString -> sl:RString -> sr:RString
  -> i:GoodIndex sl tg
  -> {v:GoodIndex (sl stringMappend sr target | v == i}

castGoodIndexLeft tg sl sr i
  = cast (subStringConcatLeft sl sr (stringLen tg) i) i
\end{code}
%
Where @cast p x@
returns @x@, after enforcing the properties of @p@ in the logic
\begin{code}
cast :: b -> x:a -> {v:a | v == x }
cast _ x = x
\end{code}
%
Moreover, the translation of @cast p x@ into the logic, is merely @x@
thus allowing random (\ie non-reflected) Haskell expressions appearing in @p@.

\paragraph{Step 2: Creation of new indices}
When concatenating two new string inputs @i1@ and @i2@,
the @stringLen tg@ last positions of @i1@ combined with the initial part of @i2@
may form new good indices.
%
@makeNewIndices s1 s2 target@ creates all such good new indices.
%
If the length of the @target@ is less than 2, then no new good indices are creates,
thus the function returns the empty list.
Otherwise, we search @concatString s1 s2@ for substring of @target@
in the range @[maxInt (stringLen s1 - (stringLen target-1)) 0, stringLen s1 - 1]@
\begin{code}
reflect makeNewIndices
makeNewIndices
  :: s1:RString -> s2:RString -> target:RString
  -> [GoodIndex {s1 stringMappend s2} target]
makeNewIndices s1 s2 target
  | lenStr target < 2
  = []
  | otherwise
  = makeIndices (s1 stringMappend s2) target lo hi
  where
    lo = maxInt (lenStr s1 - (lenStr target-1)) 0
    hi = lenStr s1 - 1
\end{code}
%
@makeIndices input target lo hi@
recursively searches for good indices on @input@ with respect to @target@
from @lo@ to @hi@.
%
\begin{code}
reflect makeIndices
makeIndices
  :: input:RString -> target:RString -> lo:Nat
  -> hi:Int -> [GoodIndex input target]
  / [hi - lo]
makeIndices input target lo hi
  | hi < lo
  = N
makeIndices input target lo hi
  | isGoodIndex input target lo
  = lo `C` rest
  | otherwise
  = rest
  where
    rest = makeIndices input target (lo + 1) hi
\end{code}
%
The notation @[hi-lo]@ declares that @makeIndices@ terminates, as the metric @hi - lo@
is a non-negative values that decreases at each recursive call.

\paragraph{Note on complexity.}
Given that the implementation of @RString@
allows substring checking via indexing, that is in constant time,
then @makeNewIndices@ and thus @(<>)@ requires @lenStr target@ checks,
that is constant checks with respect to the string input.

\paragraph{Step 3: Shift Good Indices}
If @is@ is a list of good indices for string @i2@ with respect to a target @tg@,
to get a list of good indices for the string @i1 stringMappend i2@,
we need to shift each element of @is@ @stringLen i1@ right.
%
Moreover, to persuade Liquid Haskell that the shifted indices are good indices
we need to apply the refined string theorem that states
for each string @sl@ and @sr@
and each integers @i@ and @j@,
the @subString@ on @sr@ from @i@ with length @j@
is equal to
the @subString@ on @sl stringMappend sr@ from @stringLen sl + i@ with length @j@:
%
\begin{code}
assume subStringConcatRight
  :: sl:RString -> sr:RString
  -> j:Int -> i:Int
  -> {subStr sr i j == subStr (sl stringMappend sr) (lenStr sl+i) j}
\end{code}

Thus, @shiftStringRight@ both appropriately shifts the index
and casts the shifted index using the above theorem:
\begin{code}
shiftStringRight
  :: tg:RString -> sl:RString -> sr:RString
  -> i:GoodIndex sr tg
  -> {v:(GoodIndex (sl stringMappend sr) tg) | v == i + lenStr sl}
shiftStringRight tg sl sr i
  = subStringConcatRight sl sr (stringLen tg) i)
     `cast` shift (stringLen sl) i
\end{code}


\subsection{String Matching is a Monoid}
We conclude this section by proving
that the @mempty@ and @(mappend)@
operators we defined satisfy the monoid laws.
%
In the prove, we express
\begin{itemize}
\item the monoid laws as liquid types, and
\item the monoid proofs as Haskell functions.
\end{itemize}
Then, Liquid Haskell checks that the functions indeed check the corresponding laws.

\begin{theorem}\label{theorem:monoid}
String Matching is a Monoid for the operations @mempty@ and @(mappend)@.
\end{theorem}

\begin{proof}
Based on the Monoid Definition~\ref{definition:monoid},
to prove that string maching is a monoid, we need to prove that
there exist safe implementations of the monoid laws functions.
%
We implemented the monoid laws functions
and used Liquid Haskell to (machine) check correctness of our proof.

First, we prove \textit{left identity}
\begin{code}
idLeft :: x:SM t -> {x mappend mempty == x }
idLeft (SM i is)
  =  (SM i is) mappend (mempty :: SM t)
  ==. (SM i is) mappend (SM stringMempty listMempty)
  ==. SM (i stringMappend stringMempty) (is1 listMappend isNew listMappend is2)
      ? idLeftString i
  ==. SM i (is listMappend N listMappend N)
      ? (mapCastId tg i stringMempty is &&& newIsNullLeft i tg)
  ==. SM i is
      ? idLeftList is
  ***  QED
  where
    tg    = fromString (symbolVal (Proxy :: Proxy t))
    is1   = map (castGoodIndexRight tg i stringEmp) is
    isNew = makeNewIndices i stringEmp tg
    is2   = map (shiftStringRight tg i stringEmp) N
\end{code}
The proof proceeds by rewriting and using four lemmata
\begin{itemize}
\item Left Identity on lists, that is proven by structural induction.
\begin{code}
idLeftList :: x:[a] -> {x listMappend listMempty == x}
\end{code}
\item Left Identity on strings is provided by the string library that we trust.
\begin{code}
idLeftString :: x:RString -> {x stringMappend stringMempty == x}
\end{code}
\item Identity of casting is proven by induction and identity on casts
\begin{code}
mapCastId :: tg:RString -> x:RString -> y:RString
  -> is:[GoodIndex x tg] ->
  -> {map (castGoodIndexRight tg x y) is == is}
\end{code}
\item No new indices are created by mappend
\begin{code}
newIsNullLeft :: s:RString -> t:RString
  -> {makeNewIndices s stringMempty t == listMempty }
\end{code}
The proof procceds by case splitting
on comparison of the lengths of @s@ and @t@.
At each case we prove by induction that all
the potential new indices will be out of bounds and thus
no new good indices can be created.
\end{itemize}

\NV{Actually, the right identity proof is simpler, maybe put it first}

- The proof of \textit{right identity} is similar
\begin{code}
idRight :: x:SM t -> {mempty mappend x == xs }
idRight (SM i is)
  =  (mempty :: SM t) mappend (SM i is)
  ==. (SM stringMempty listMempty) mappend (SM i is)
  ==. SM (stringMempty <+> i) (is1 ++ isNew ++ is2)
       ? idRightString i
  ==. SM i (N ++ N ++ is)
       ? (mapShiftZero tg i is &&& newIsNullRight i tg)
  ==. SM i is
       ? idRightList is
  *** QED
  where
    tg    = fromString (symbolVal (Proxy :: Proxy t))
    is1   = map (castGoodIndexRight tg i stringEmp) N
    isNew = makeNewIndices stringEmp i tg
    is2   = (map (shiftStringRight tg stringEmp i) is)
\end{code}
The proof uses again four lemmata.
\begin{itemize}
\item Right Identity on lists, that is proven by structural induction.
\begin{code}
idRightList :: x:[a] -> {listMemtpy listMappend x == x}
\end{code}
\item Right Identity on strings is provided by the string library that we trust.
\begin{code}
idRightString :: x:RString -> {stringMemepty stringMappend x == x}
\end{code}
\item Identity of shifting by an empty string is proven by induction and
the assumption that empty string has length 0
\begin{code}
mapShiftZero :: tg:RString -> i:RString -> is:[GoodIndex i target]
  -> {map (shiftStringRight tg stringMempty i) is == is }
\end{code}
\item No new indices are created by mappend
\begin{code}
newIsNullLeft :: s:RString -> t:RString
  -> {makeNewIndices stringMempty s t == listMempty }
\end{code}
The proofs relies on the fact that @makeIndices@
will be called on the range @[0, -1]@ and immediately return @listMemepty@.
\end{itemize}
- Finally we prove \textit{associativity}.
For space, we omit the detailed proof, and only give the interesting steps.
In the proof we need to show equality of two string matchers,
thus we need to show that their input and induces fields are respectively equal.
%
Equality of the input fields follows by associativity of RStrings.
%
The proof of index equlity proceeds in three steps.

\begin{enumerate}
\item Firstly, using list associativity and distribution of index shifting,
we group the indices in the five lists shown in Figure~\ref{fig:mappend:assoc}.
The indices of the input @x@,
the new indices from mappending @x@ to @y@,
the indices of the input @y@,
the new indices from mappending @x@ to @y@, and
the indices of the input @z@.
\item The representation of each group depends on the order of appending.
For example, if @zis1@ (resp. @zis2@) is the group @zis@ when
right (resp. left) mappend happened first, then we have
\begin{code}
zis1 = map (shiftStringRight tg xi (yi stringMappend zi))
       map (shiftStringRight tg yi zi) zis

zis2 = map (shiftStringRight tg (xi stringMappend yi) zi) zis
\end{code}
That is, in right first, the indices of @z@ are first shifted
by the length of @yi@ and then by the length of @xi@,
while in the left first case, the indices of @z@ are shifted by the
length of @xi stringMappend yi@.
In this second step of the proof, we prove using lemmata,
the equivalence of the group representation.
Equivalence of @xis@ and @zis@ is trivial,
but for the rest three groups, as we later discuss is more interesting,
as it depends on the relative lengths of the target and the input of @y@.
\item Finally, once we proved equivalence of representations,
we use again list associativity and distribution of casts to wrap the index groups
back in string matchers
\end{enumerate}
\begin{figure}
\includegraphics[scale=0.5]{AssociativeIndices}
\label{fig:mappend:assoc}
\end{figure}
Bellow we present the skeleton of the proof, while the detailed proof can be found online\footnote{\NV{GIVE PRoof link}}.
\begin{code}
assoc x@(SM xi xis) y@(SM yi yis) z@(SM zi zis)
  -- Step 1: unwrapping the indices
  =   x <> (y <> z)
  ==. (SM xi xis) <> ((SM yi yis) <> (SM zi zis))
                         ...
  -- via list associativity and distribution of shifts

  -- Step 3: Equivalence of representations
  ==. SM i (xis1 ++ ((xyis1 ++ yis1 ++ yzis1) ++ zis1))
  ==. SM i (xis1 ++ ((xyis1 ++ yis1 ++ yzis1) ++ zis1))
      ? castConcat tg xi yi zi xis
  ==. SM i (xis2 ++ ((xyis1 ++ yis1 ++ yzis1) ++ zis2))
      ? mapLenFusion tg xi yi zi zis
  ==. SM i (xis2 ++ ((xyis2 ++ yis2 ++ yzis2) ++ zis2))
      ? assocNewIndices y tg xi yi zi yis

  -- Step 3: Wrapping the indices
                         ...
  -- via list associativity and distribution of casts
  ==. (SM xi xis <> SM yi yis) <> SM zi zis
  =   (x <> y) <> z
  *** QED
  where
    yzis1 = map (shiftStringRight tg xi (yi <+> zi)) yzis
    yzis2 = makeNewIndices (xi <+> yi) zi tg

    yzis  = makeNewIndices yi zi tg

    i     = xi stringMappend (yi stringMappend zi)
\end{code}
Finally, we present the lemma @assocNewIndices@
that proofs equivalence of representation in the three
groups @xyis@, @yis@, and @yzis@.
The proof proceeds by case analysis in the relative size of
the target @tg@ and the middle input @yi@.
%
If the target is smaller than @yi@
then we can prove equivalence of each of the groups independently
via respective lemmata.
%
Otherwise, independent equivalence does not hold.
Thus, when @yi@ is smaller than the target,
the group @xyis1@ (similarly @yzis1@)
is not provably equal to @xyis2@ (similarly @yzis2@).
When @yi@ is smaller than the target,
when appending @x@ with @y mappend z@ new indices may occur because
of the suffix of @z@, these indices will not occur when appending @x@ with @y@.
%
Yet, the appending of the two new index groups are provably equal,
@xyis1 listMappend yzis1 == xyis2 listMappend yzis2@.
The lemma proof using append equivalence and the fact @yis1 == yis2 == []@
to conclude that the appending of all the three groups is always equivalent.

\begin{code}
-- proof that
-- xyis1 ++ yis1 ++ yzis1 == xyis2 ++ yis2 ++ yzis2
assocNewIndices y tg xi yi zi yis
  | stringLen tg <= stringLen yi
  =   xyisEquivalence xi yi zi tg
  &&&  yisEquivalence xi yi zi tg yis
  &&& yzisEquivalence xi yi zi tg
  | stringLen yi < stringLen tg
  =  xyis1 listMappend yis1 listMappend yzis1
  ==. xyis1 listMappend [] listMappend yzis1 ? emptyIndices y yis
  ==. xyis1 listMappend yzis1 ? idLeftList xyis1
  ==. xyis2 listMappend yzis2 ? shiftNewIndices xi yi zi tg
  ==. (xyis2 listMappend []) listMappend yzis2 ? idLeftList xyis2
  ==. (xyis2 listMappend yis2) listMappend yzis2 ? emptyIndices y yis
  *** QED
\end{code}


\qed\end{proof}


==> overview.tex <==
\section{Overview}\label{sec:overviews}

\def\sm{\texttt{sm}}
\def\mc{\texttt{mconcat}}

\subsection{Monoids and Parallelism}\label{subsec:monoids}

As noted in section~\ref{sec:intro}, associativity ultimately
allows monoidal operations to be run in parallel. However, for our
purposes, we would like a way of breaking an input into pieces and
running our computation, string matching, in parallel on all the
pieces. For this, we will focus on the standard Haskell function \mc,
\begin{code}
  mconcat :: Monoid m => [m] -> m
  mconcat [] = mempty
  mconcat (x:xs) = x <> mconcat xs
\end{code}
where @mappend@ and @mempty@ are the monoid operation and identity for
monoid \texttt{m} (usually written \texttt{mappend} and
\texttt{mempty})~\footnote{\mc\, is usually defined as \texttt{foldr mappend mempty}}.

\mc is a monoid morphism from lists of values of
a monoid to that monoid, i.e.
%
$$
\begin{array}{rcl}
\mc\;[] & \quad \equiv \quad & \mempty \\
\mc\;([x_0,\;\ldots x_m]\;\texttt{++}\;[y_0,\ldots y_n])
& \quad \equiv \quad &
\mc\;[x_0, \ldots x_m]\;\mappend\;\mc\;[y_0,\ldots y_n]
\end{array}
$$
%
where \texttt{++} is list append.

$$
\begin{array}{l}
\mc\;[\sm\;x_0,\;\ldots \sm\;x_i, \sm\;x_{i+1},\ldots \sm\;x_j, \sm\;x_{j+1},\ldots \sm\;x_n] \\
\;\;\equiv\;\; \quad
\mc\;([\sm\;x_0,\;\ldots \sm\;x_i]\;\texttt{++}\;[\sm\;x_{i+1},\ldots \sm\;x_j]\;\texttt{++}\;[\sm\;x_{j+1},\ldots \sm\;x_n]) \\
\;\;\equiv\;\; \quad
%\mc\;[\mc\;[\sm\;x_0,\;\ldots \sm\;x_i]\;,\;\mc\;[\sm\;x_{i+1},\ldots \sm\;x_n]] \\
%\;\;\equiv\;\; \quad
\mc\;[\sm\;x_0, \ldots \sm\;x_i]\;\mappend\;\mc\;[\sm\;x_{i+1},\ldots \sm\;x_j]\;\mappend\;\mc\;[\sm\;x_{j+1},\ldots \sm\;x_n]
\end{array}
$$


\subsection{String Matching}\label{subsec:string-matching}

String matching is determining all the indices in a source string
where a given target string begins; for example, for source string
\texttt{abababa} and target \texttt{aba} the results of string
matching would be \texttt{[0, 2, 4]}. We will use the following code
as a specification of string matching:
\begin{code}
makeIndices inp trg = go 0 where
  trgLen = length trg
  go i | i >= length inp = []
       | take trgLen (drop i inp) == trg = i : rest
       | otherwise = rest
  where rest = go (i + 1)

*Main> makeIndices "abababa" "aba" == [0, 2, 4]
\end{code}
Though this implementation is not efficient, it is simple and provides
a good starting point from which to create a verifiable function (see
sec~\ref{sec:monoid}).

\subsection{Monoidal String Matching}\label{subsec:monoidal-string-matching}


==> parallelization.tex <==
\section{Verification of Parallel Concatenation on Monoids}\label{sec:parallelization}
In this section we define how to concatenate a list of monoids
into a monoid. 
%
Then, we parallelize list concatenation 
and use LiquidHaskell to prove that the 
parallel and sequential versions are equivalent. 
\NV{What does equivalence means here?}

\subsection{Concatenation of lists using monoids}
If @m@ is a monoid, then @mconcat@ reduces a list of monoids @xs@
to one monoid. 
\begin{code}
mconcat :: List m -> m 
mconcat N        = mempty
mconcat (C x xs) = x mappend (mconcat xs)
\end{code}
%
Concatenation folds the elements of the list using @(mappend)@ 
and returns @mempty@ when the list is empty. 

Next, we define a parallel version of list concatenation 
%
\begin{code}
pmconcat :: Int -> List m -> m
pmconcat i xs  | i <= 1 || llen xs <= i
  = mconcat xs 
pmconcat i xs 
  = pmconcat i $ withStrategy parStrategy $  
                 map mconcat (chunk i xs)
\end{code}%$
The function @pmconcat i xs@ calls @mconcat xs@ in the base case, 
otherwise it
(1) chunks the list @xs@ in lists of size @i@, 
(2) runs in parallel @mconcat@ to each chunk, 
(3) recursively runs itself in the result list.
%
Termination of @pmconcat@ holds, as the length of @chunk i xs@
is smaller than the length of @xs@, when @1 < i@. 
%
Concretely, we define @chunk@ using the standard definition for 
list @take@ and @drop@.
\begin{code}
chunk :: i:Pos -> xs:List a 
  -> {v:List (List a) | chunkRes i xs } 
chunk i xs 
  | length xs <= i 
  = C xs N 
  | otherwise
  = C (take i xs) (chunk i (drop i xs))

chunkRes i xs
  | length xs <= i = length v == 1 
  | i == 1         = length v == length xs
  | otherwise     = length v < length xs
\end{code}

Where @take@ and @drop@ type as follows
\begin{code}
drop :: i:Nat -> xs:{List a | i <= length xs } 
  -> {v:List a | length v == length xs - i }
take :: i:Nat -> xs:{List a | i <= length xs } 
  -> {v:List a | length v == i }
\end{code}


\paragraph{Runtime Parallelism.}
To parallelize concatenation of the chunks we use parallel strategies 
from the Haskell library @Control.Parallel.Strategies@.
%
For example, in our implementation @parStrategy@ is defined as
\begin{code}
parStrategy :: Strategy (List a)
parStrategy = parTraversable rdeepseq
\end{code}

Note that parallelization of concatenation leads to runtime speedups
only when @(mappend)@ runs in constant time with respect to the monoid size. 
%
Otherwise, at each recursive call of @pmconcat@,
runtime will be dominated by the size of the biggest list element. 

Even though runtime of the parallel version depends on the implementation details 
of the monoids, correctness holds for every monoid. 
%
In the rest of this section we prove equivalence of the sequential and parallel concatenation operations. 


\paragraph{Parallelism in the Logic.}
To prove equivalence we make the \textit{assumption}
that the Haskell function @withStrategy s x@ 
returns @x@ for every strategy.
\begin{code}
assume withStrategy :: Strategy a -> x:a -> {v:a | v == x}
\end{code}
%
Moreover, to prove equivalence, we need to represent 
the implementation of @pmconcat@ in logic.
%
Which, in turn, requires representation of @withStrategy@. 
%
LiquidHaskell represents @withStrategy@ in logic as a function that merely returns
its second argument @withStrategy _ x = x@
and does not reason about parallelism. 

\subsection{Equivalence of Parallel and Sequential Concatenation}

\begin{theorem}[Monoid Concatenation Equivalence]\label{theorem:equivalence:concat}
If @m@ is monoid, then the parallel and sequential concatenations are equivalent:
\begin{code}
pmconcatEquivalence 
  :: i:Int -> is:List m -> { pmconcat i is == mconcat is }
\end{code}
\end{theorem}

\begin{proof}
We prove the theorem by providing a Haskell implementation of @pmconcatEquivalence@
that is safe under LiquidHaskell. The details of the proof can be found in~\cite{implementation}, 
here we provide the sketch of the proof. 

First we prove that @mconcat@ distributes over list splitting
\begin{code}
mconcatSplit 
  :: i:Nat -> xs:{List m | i <= llen xs} 
  -> { mconcat xs == mconcat (take i xs) 
                 <> mconcat (drop i xs) }
\end{code}
%
The proofs proceeds by structural induction, using monoid left identity in the base case
and associavity in the inductive step.

We generalize the above lemma
to prove that @mconcat@ distributes over list chunking
\begin{code}
mconcatChunk 
  :: i:Pos -> xs:List (Monoid a) 
  -> { mconcat xs == mconcat (map mconcat (chunk i xs)) }
\end{code}
%
The proofs proceeds by structural induction, using monoid left identity in the base case
and lemma @mconcatSplit@ in the inductive step.

Lemma @mconcatChunk@ is sufficient to prove @pmconcatEquivalence@ by structural induction, 
using monoid left identity in the base case. 
\qed\end{proof}

Note that the proof uses only the monoid laws and not the implementations of the monoid
operators, thus the theorem holds \textit{for any} type that satisfies the monoid laws. 
%
Next we define a monoid structure for string matching and prove it satisfies the monoid laws. 
Thus we conclude that string matching concatenation can be parallelized. 
 


==> strings.tex <==
\section{Refined Strings}\label{sec:strings}

Refined Strings provides a wrapping over a string manipulations library, 
here `ByteString`
\begin{code}
data RString = S BS.ByteString 
\end{code}

String operators wrap the library operators
and moreover they are assumed to be reflected into the logic

\begin{code}
assume concatString :: x:LHString -> y:LHString 
      -> {v:LHString | v == concatString x y }
concatString (S s1) (S s2) = S (s1 `BS.append` s2)

assume stringEmp :: {v:RString | v == stringEmp  && stringLen v == 0 } 
stringEmp = S (BS.empty)

assume stringLen :: x:RString -> {v:Nat | v == stringLen x}
stringLen (S s) = BS.length s 

assume subString  :: s:RString -> offset:Int -> ln:Int -> {v:RString | v == subString s offset ln }
subString (S s) o l = S (BS.take l (BS.drop o s))

assume takeString :: i:Nat -> xs:{RString | i <= stringLen xs } 
  -> {v:RString | stringLen v == i && v == takeString i xs }
takeString i (S s) = S (BS.take i s)

assume dropString :: i:Nat -> xs:{RString | i <= stringLen xs } 
  -> {v:RString | stringLen v == stringLen xs - i && v == dropString i xs }
dropString i (S s) = S (BS.drop i s)

assume fromString :: i:String -> {o:RString | i == o && o == fromString i}
fromString = S . ST.fromString 

assume isNullString :: i:RString -> {b:Bool | Prop b <=> stringLen i == 0 }
isNullString (S s) = BS.length s == 0 
\end{code}


Finally the refined string library, exposes theorems that hold (but are assumed) 
for the internal string representation

\begin{code}
assume stringEmpProp :: x:RString  -> { stringLen x == 0 <=> x == stringEmp }
stringEmpProp _ = trivial 
 
assume concatStringNeutralLeft :: x:RString -> {concatString x stringEmp == x}
concatStringNeutralLeft _ = trivial

assume concatStringNeutralRight :: x:RString -> {concatString stringEmp x == x}
concatStringNeutralRight _ = trivial

assume concatTakeDrop :: i:Nat -> xs:{RString | i <= stringLen xs} 
    -> {xs == concatString (takeString i xs) (dropString i xs) }
concatTakeDrop _ _ = trivial

assume concatLen :: x:RString -> y:RString -> { stringLen (concatString x y) == stringLen x + stringLen y }
concatLen _ _ = trivial

assume concatStringAssoc :: x:RString -> y:RString -> z:RString 
     -> {concatString (concatString x y) z == concatString x (concatString y z) }
concatStringAssoc _ _ _ = trivial


-- | Substrings 

assume subStringConcatBack :: input:RString -> input':RString -> j:Int -> i:{Int | i + j <= stringLen input }
  -> { (subString input i j == subString (concatString input input') i j) }
subStringConcatBack _ _ _ _ = trivial  


assume subStringConcatFront  
  :: input:RString -> input':RString -> j:Int -> i:Int 
  -> { (subString input i j == subString (concatString input' input) (stringLen input' + i) j) }
subStringConcatFront _ _ _ _ = trivial
\end{code}
